An Efficient Sliding Mesh Interface Method for High-Order Discontinuous Galerkin Schemes

Sliding meshes are a powerful method to treat deformed domains in computational fluid dynamics, where different parts of the domain are in relative motion. In this paper, we present an efficient implementation of a sliding mesh method into a discontinuous Galerkin compressible Navier-Stokes solver and its application to a large eddy simulation of a 1-1/2 stage turbine. The method is based on the mortar method and is high-order accurate. It can handle three-dimensional sliding mesh interfaces with various interface shapes. For plane interfaces, which are the most common case, conservativity and free-stream preservation are ensured. We put an emphasis on efficient parallel implementation. Our implementation generates little computational and storage overhead. Inter-node communication via MPI in a dynamically changing mesh topology is reduced to a bare minimum by ensuring a priori information about communication partners and data sorting. We provide performance and scaling results showing the capability of the implementation strategy. Apart from analytical validation computations and convergence results, we present a wall-resolved implicit LES of the 1-1/2 stage Aachen turbine test case as a large scale practical application example.

==> 1.tex <==
\section{Introduction}
\label{sec:introduction}







High-order methods have significantly gained popularity over the last decade, due to their potential advantages in terms of accuracy and efficiency for many applications \cite{wang2013}. A variety of high-order schemes has been proposed in literature, such as the WENO schemes \cite{liu1994,balsara2000}, the flux reconstruction method \cite{huynh2007} and the spectral difference method \cite{liu2006,wang2007}, with the latter two also being closely related to the Discontinuous Galerkin (DG) methods \cite{may2011,degrazia2014}. In particular the Discontinuous Galerkin Spectral Element Method (DGSEM) \cite{hesthaven2007,hindenlang2012} has shown its suitability for simulations of unsteady turbulent flows in large-scale applications and high-performance computing (HPC) as consequence of its high-order of accuracy as well as its excellent scaling properties \cite{atak2016,beck2014high,bolemann2015high,wang2013high}. While the development of novel formulations and efficient schemes is still ongoing, there is sufficient evidence from published results that DG and related methods have reached a certain level of maturity. Thus, adding and exploring new the features to the existing formulations - while retaining the original properties - has now become another focus of ongoing development. Examples of this include the integration of shock capturing mechanism, \\
However, many fields of engineering interest, as e.g. turbomachinery, wind turbines and rotorcraft, are characterized by moving geometries and large periodic displacements. A common technique to incorporate this movement into numerical schemes is the arbitrary Lagrangian-Eulerian (ALE) approach \cite{minoli2011}, which introduces a time-dependent mapping from an arbitrarily deformed domain to the undeformed reference state. Since the mesh connectivity remains unchanged, this approach is often limited to small relative displacements.
In the sliding mesh method \cite{van2006,bakker1997,jaworski1997,ng1998,mcnaughton2014}, the computational domain is divided into subdomains, which can slide along a common interface while preserving the mesh geometry inside each subdomain.  
The overset mesh (Chimera) method \cite{wang2014,ahmad1996,pomin2002,sankaran2011,zahle2009} employs several independent meshes inside the computational domain, which can be moved independently and are coupled by means of the overlapping regions.
Schematics of the discussed methods are shown in \figref{fig:MovingMesh}. \todo{Examples for (low-order) methods or better for applications?}
\begin{figure}[htb]
	\centering
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=0.6\textwidth]{fig/ALE.eps}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=0.6\textwidth]{fig/SlidingMesh.eps}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\centering
		\includegraphics[width=0.6\textwidth]{fig/Chimera.eps}
	\end{subfigure}
	\caption{Common moving mesh techniques: the arbitrary~Lagrangian-Eulerian~approach~(ALE)~(\textit{left}), the~sliding~mesh~method (\textit{middle}) and the overset~mesh or Chimera method (\textit{right})}
	\label{fig:MovingMesh}
\end{figure}

However, these methods generally do not retain the high-order of accuracy of the underlying numerical scheme, wherefore special interest is brought to high-order accurate variants of these moving mesh methods, e.g. the sliding mesh method \cite{zhang2015,zhang2016,qiu2019,ferrer2012,ramirez2015} or the Chimera method \cite{wurst2015,brazell2016}.
To this end, we propose an efficient implementation and parallelization strategy for the sliding mesh method introduced by Zhang and Liang \cite{zhang2015}, which preserves the high-order accuracy of DGSEM and retains the excellent scaling properties of the baseline code for massively parallel large-scale applications.\\
The outline of this paper is as follows. The governing equations on the moving domain are given in \secref{sec:equations} and the DGSEM scheme as well as the treatment of non-conforming meshes are discussed in \secref{sec:numerics}. \secref{sec:implementation} gives details on the proposed implementation and parallelization strategy for the sliding mesh method. The results in \secref{sec:results} entail the convergence of the method, its scaling properties and the suitability for large-scale applications. To this end, an implicit large eddy simulation (LES) of the 1-1/2 stage turbine test case \textit{Aachen Turbine} has been carried out. \secref{sec:conclusion} concludes the paper.


==> Makefile <==
FILENAME='sm_paper'

all:
	rubber -f --pdf -s --synctex --warn=all --jobname=$(FILENAME) $(FILENAME).tex

clean:
	ls *.tex | rev | cut -c 5- | rev | xargs rubber --clean


run:
	nohup okular --unique $(FILENAME).pdf\#src:$(LINE)$(FILE) &

